rTisane: Externalizing conceptual models for data analysis increases engagement with domain knowledge and improves statistical model quality

Statistical models should accurately reflect analysts' domain knowledge about variables and their relationships. While recent tools let analysts express these assumptions and use them to produce a resulting statistical model, it remains unclear what analysts want to express and how externalization impacts statistical model quality. This paper addresses these gaps. We first conduct an exploratory study of analysts using a domain-specific language (DSL) to express conceptual models. We observe a preference for detailing how variables relate and a desire to allow, and then later resolve, ambiguity in their conceptual models. We leverage these findings to develop rTisane, a DSL for expressing conceptual models augmented with an interactive disambiguation process. In a controlled evaluation, we find that rTisane's DSL helps analysts engage more deeply with and accurately externalize their assumptions. rTisane also leads to statistical models that match analysts' assumptions, maintain analysis intent, and better fit the data.

==> archive/discussion-old.tex <==
\section{Discussion}
Try to match these to contributions??

\subsection{What we know about data analysis praxis}
Hypothesis formalization process
- Using hypothesis formalization as a lens for interpreting the results from the qual lab study and evaluation....
- Do these findings suggest updates to our model of hypothesis formalization?

\subsection{Design  methods}
Co-design DSL + UI + statistics engine

Syntax is easier to design for usability
- straightforward barrier to adopting a language or tool
- current methods make pribing into and iterating on syntax easier, probing into semantics is harder. 
- However, experiences and preferences for syntax can highly contaminate/bias findings such that we are used to the syntax of popular languages
We run into similar concerns with semantics, but by targeting novices we can overcome some of the fixation on previous experiences. (We see it in the "if I were to write a statistical model" framework rather than an entirely new/different programming paradigm/model where people dont write the model directl themselves.)
Punchline: Semantics is necessary because it has an impact on problem formulation, solution engineering, and ultimately, we believe, relevance to the domain (it could be super usable syntactically, but if the DSL doesnt contain the primitives that end-users can grasp onto and use, the language and tool doesnt solve the problem). 
Therefore, we study semantics. 

Design process/methods: Ways of approximating internalized semantics.
Tea - Stats courses
Tisane - Experimental design libraries and tools, some feedback from researchers 
rTisane - start with users to elicit semantics
rTisane required an existing OSS Tisane to use as a probe, so in some ways, this method is the natural consequence of other attempts to approximate semantics.

Add nuance to the current discussion in PLIERS for how to come up with semantics, which is largely left up to the language designer in existing methodological frameworks.

Language - Interaction -- usable programming

\textit{Bottom-up specification}
- bottom-up approach
- role of statistical analysis tools for educating on statistical concepts - promising direction is to imbue our tools with greater automation and intelligence but with approachable explanations and ideas (connect to AI interpretability?)



\textit{Summative evaluation conditions + ecological validity}
Some may argue that a more ecologically study design would have compared rTisane
with no help, not even a scaffolded workflow. We opted for a higher ``baseline''
in the control condition because we wanted to assess the influence of tooling on
connecting conceptual modeling to statistical modeling. We would expect that
this alternative design would show that rTisane has a larger influence on
improving statistical models.


\textit{Open question in causal reasoning community -- how to get domain experts who are not statistical/causal experts to express causal diagrams}

\textit{Current ecosystem of tools that ignore conceptual modeling}
While some analysts may externalize
their domain knowledge through informal graphs or statements of variable
relationships, expressing and grappling with conceptual knowledge in the context
of statistical analysis is largely ignored in existing statistical analysis
tools. In the current ecosystem, tools for expressing conceptual models exist
but are separate from those used for authoring and executing statistical models,
which tend to be focused on the mathematical formulations of statistical models,
ignoring the conceptual meaning behind them. This division may, in fact,
contribute to inconsistencies between conceptual knowledge and statistical
models. 


Conceptual models are difficult to reason about during statistical analysis
because they involve implicit assumptions whose correspondence to data and 
implications on statistical modeling are not obvious, especially to
statistical non-experts. For example, the impact of conceptual assumptions may only
become apparent after fitting statistical models. Many iterations of
statistical analyses are actually refinements to the conceptual models they are
supposed to represent. Without explicitly grappling with conceptual models prior
to authoring statistical models, analysts run the risk of introducing
inconsistencies between their domain knowledge and statistical models, which can
lead to unintentionally answering a different research question, and opening
themselves up to HARKing (asserting a conceptual model based on preferred
results). 

Together, \rTisane's specification language and reasoning engine scaffold the
statistical model authoring process, shifting the burden of statistical model
expertise from users to software while focusing analysts on their conceptual
goals and implicit assumptions. 

==> archive/generating_data.tex <==
The outcome should be normally distributed...

==> archive/glm_study.tex <==
% \ej{Note: Having two separate studies, one for GLM and another for GLMMS, offers (i) a simpler study design compared to one monolithic study and (ii) provides us with an opportunity to potentially tweak the design/tasks/interview questions between studies.}

\section{Study 1: Evaluating the impact of Tisane on authoring GLMs}
We conducted a within-subjects think-aloud study comparing Tisane to existing
tools for authoring generalized linear models. We focused our study on the
following research questions: 
\begin{itemize}
    \item Does Tisane help analysts avoid mistakes in specifying their models? 
    \item Can Tisane help analysts learn more about their data and methods? 
\end{itemize}

\subsection{Participants}
We recruited \ej{N} participants through mailing lists, word of mouth, and
statistics-focused discussion fora \ej{(will need to generate concrete list)},
and Upwork. We determined this sample size based on a priori statistical power
calculations. \ej{Planning to explore sample sizes and statistical power.}

The only criteria for participation in the study was that participants had to report
having experience with linear models. \ej{Participants had X median years of
experience (mean, std). P\% of participants were very or somewhat familiar with
using Python to author linear models. Q\% participants were very or somewhat
familiar with R for authoring linear models. Some participants had never used
Python or R but instead preferred Stata (\%), SPSS(\%), etc. None had used or
heard of Tisane before....} 

\ej{I plan to include a pre-survey to determine
elligibility while recruiting. I only plan to filter based on experience and
maybe current country location if there is a rule about recruitment/payment.
Need to double check UW rules.}

\subsection{Protocol}
\ej{I'm debating if we should conduct the study via Zoom or in-person. Conducting an in-person study would eliminate installation issues but might restrict the participant pool too much.}

The study was conducted remotely via Zoom. At the beginning of the study, the
researcher gave an overview of the study. Each participant analyzed two datasets
on (i) \ej{the demographic influences of income, which was based on [a study the
Pew Research Center conducted in 2014?],} and (ii) \ej{the effects of tutoring on
test achievement, which was based on XX}.

We asked participants to analyze one dataset using Tisane and the other using
any other tool(s) they wanted. For each dataset, we gave participants the
dataset in a CSV, a summary of the data schema, and \ej{a summary of the causal
model - not sure about this}. We counterbalanced the order of datasets and tools
across participants. For each dataset, analysts were asked to answer \ej{K}
questions that required them to author, report, and interpret generalized linear
models. The order of analysis question for each dataset was randomized for each
participant. Participants were given 30 minutes to explore and analyze each
dataset. After half an hour, we asked participants to stop.

Before using Tisane, the researcher guided participants through installation, a tutorial, and
two examples, which took approximately 20 minutes. Participants could also
freely explore other examples in Tisane's open source repository prior to
feeling familiar enough with Tisane to begin analyzing a dataset. Participants
spent an average of \ej{M} minutes learning to use Tisane. 

% Although we
% did not have an explicit research question about how easy or diffuclt Tisane was
% to use for the first time, p

After analyzing both datasets, participants completed a post-survey that asked
about their domain expertise, analysis backgrounds, familiarity with the domains represented in the
datasets, how their expected and actual findings compared, and the impact of
their expectations on how they explored or trusted the data, models, and
results. Finally, in a semi-structured exit interview, the researcher asked
participants about any uncertainties or doubts they had doing their analyses and
any takeaways or lessons they learned throughout the process of using Tisane.
With participant consent, we recorded participants' screens, video, and audio
throughout the study. The lab session lasted approximately 90 mintues, and
participants were compensated \$25 for their time. 

\ej{Maybe we want to include a few NASA-TLX questions to assess task difficulty after each dataset-tool combo as well?}

\subsection{Materials}
% \ej{Large portions of this section should be in an appendix instead of the body
% of the paper. For a more streamlined reading experience, I have placed all the
% details here.} 
% \subsubsection{Dataset generation}
\ej{Some of this is likely to change as I iterate on datasets.}
To have ground truth statistical models, we simulated both datasets. We started
from causal models based on those presented in research papers about
income~\ej{\cite{}} and education~\ej{\cite{}}. When simulating the datasets, we
ensured the causal models and variables exhibited properties (e.g., confounding,
categorical data types) where common modeling mistakes would lead to incorrect
statistical models and results. 

We identified the following modeling mistakes from textbooks
(McElreath~\cite{mcelreath2020statistical} Gelman and
Hill~\cite{gelmanHill2006regression}; and Cohen, Cohen, West, and
Aiken~\cite{cohen1988statistical}): 
\begin{enumerate}
    \item Omitting an important variable that would change the magnitude and statistical significance of coefficients of all other variables
    \item Multicollinearity: Including unnecessary variables that change the magnitude and statistical significance of all other variables [not sure how to simulate this yet]
    \item Omitting an interaction that would change the magnitude and statistical significance of all other coefficients
    \item Assuming Gaussian/identity link (linear regresion) inappropriately
    \item Using a log transform leads to different results as when using a log link function [not sure how to siumlate this yet]
\end{enumerate} 

We developed \ej{Q} analysis questions (1 per mistake) intentionally designed to lead
participants to erroneous models without careful consideration. We included an
open-ended analysis question that was always at the very end to contrast how
participants may analyze the dataset more freely.

\ej{Include the causal models, analysis questions, answers to the questions as supplementary material.}

\subsection{Measures}
\textit{Error:} For each analysis question, we first determined if the
participant discovered the ground truth model (binary outcome). If not, we
quantified the severity of the error as the difference in \textbf{model fit}
(i.e., AIC, BIC, Adjusted R-squared), the \textbf{coefficients} for each
variable (i.e., the signs of coefficients and the absolute values/relative
magnitudes of coefficients), and the \textbf{uncertainty} associated with each
variable (i.e., standard errors, confidence intervals, and p-values).

In a qualitative analysis, we (i) identified the observable error (e.g., exclude a key
variable) in the submitted model and (ii) conducted a root cause analysis from
the recorded audio and video traces. We looked for the chain of assumptions and
decisions that led to the error. To identify common sources of error, we
compared the chains of actions leading to observed errors across participants.

\ej{Should the root cause analysis be conducted with the participant at the end lab study or in a follow-up session? Rather than among the researchers afterwards?}

% The researcher also asked follow-up questions
% in the closing interview to probe into the analysts' rationale for each observed
% error. 

\textit{Learning:} We thematically analyzed participants' responses to the
post-survey and semi-structured interview questions about what they learned
about their data and analytical approaches from their experience using Tisane.

\ej{Should we ask about what they learned from their analyses without Tisane?}

\subsection{Findings}
\ej{TBD!}

\subsection{Discussion}
\ej{Update this once I have read up on related work on error classification systems...}
For errors, we should relate the observed chains and observed errors to Norman's
model of error (slips vs. mistakes); Rasmussen's modes of behavior (skill vs.
rule vs. knowledge); hypothesis formalization (?).

==> archive/glmm_study.tex <==
\section{Study 2: Evaluating the impact of Tisane on authoring GLMMs for hierarchical data and repeated measures}
\ej{Studies 2 and 3 are very similar to Study 1. I have highlighted in blue the places \diff{where Study 2/3 differ from Study 1.}}

We conducted a within-subjects think-aloud study comparing Tisane to existing
tools for authoring generalized linear models \diff{with mixed-effects}. We focused our study on the
following research questions: 
\begin{itemize}
    \item Does Tisane help analysts avoid mistakes in specifying their \diff{mixed-effects} models? 
    \item Can Tisane help analysts learn more about their data and methods? 
\end{itemize}

\subsection{Participants}
We recruited \ej{N} participants through mailing lists, word of mouth, and
statistics-focused discussion fora \ej{(will need to generate concrete list)},
and Upwork. We determined this sample size based on a priori statistical power
calculations. \ej{Planning to explore sample sizes and statistical power.}

The only criteria for participation in the study was that participants had to report
having experience with \diff{mixed-effects} linear models. \ej{Participants had X median years of
experience (mean, std). P\% of participants were very or somewhat familiar with
using Python to author linear models. Q\% participants were very or somewhat
familiar with R for authoring linear models. Some participants had never used
Python or R but instead preferred Stata (\%), SPSS(\%), etc. None had used or
heard of Tisane before....} 

\ej{I plan to include a pre-survey to determine
elligibility while recruiting. I only plan to filter based on experience and
maybe current country location if there is a rule about recruitment/payment.
Need to double check UW rules.}

\ej{\subsection{Protocol}} The study was conducted remotely via Zoom. At the
beginning of the study, the researcher gave an overview of the study. Each
participant analyzed two datasets: (i) \ej{the demographic influences of income
within families over five years, which was based on XX} and (ii) \ej{the effects
of tutoring on monthly test achievement throughout the school year, adapted from
XX}. Both datasets contained hierarchies (i.e., individuals within families,
students within classrooms) as well as repeated meaures (i.e., over five years,
over the school year), two types of study designs and datasets that
necessitate mixed effects. 
% ; and (iii) \ej{the effects of syntax on lexicographic discrimination (non-nesting composition),
% adapted from~\cite{barr2013random}}. 

We asked participants to analyze one dataset using Tisane and the other using
any other tool(s) they wanted. For each dataset, we gave participants the
dataset in a CSV, a summary of the data schema, and \ej{a summary of the causal
model - not sure about this}. We counterbalanced the order of datasets and tools
across participants. For each dataset, analysts were asked to answer \ej{K}
questions that required them to author, report, and interpret generalized linear
models. The order of analysis question for each dataset was randomized for each
participant. Participants were given 30 minutes to explore and analyze each
dataset. After half an hour, we asked participants to stop.

Before using Tisane, the researcher guided participants through installation, a tutorial, and
two examples, which took approximately 20 minutes. Participants could also
freely explore other examples in Tisane's open source repository prior to
feeling familiar enough with Tisane to begin analyzing a dataset. Participants
spent an average of \ej{M} minutes learning to use Tisane. 

% Although we
% did not have an explicit research question about how easy or diffuclt Tisane was
% to use for the first time, p
After analyzing both datasets, participants completed a post-survey that asked
about their domain expertise, \diff{analysis background including how familiar they were with mixed effects models}, familiarity with the domains represented in the
datasets, how their expected and actual findings compared, and the impact of
their expectations on how they explored or trusted the data, models, and
results. Finally, in a semi-structured exit interview, the researcher asked
participants about any uncertainties or doubts they had doing their analyses and
any takeaways or lessons they learned throughout the process of using Tisane.
With participant consent, we recorded participants' screens, video, and audio
throughout the study. The lab session lasted approximately 90 mintues, and
participants were compensated \$25 for their time. 

\ej{Maybe we want to include a few NASA-TLX questions to assess task difficulty after each dataset-tool combo as well?}

\subsection{Materials}
% \ej{Large portions of this section should be in an appendix instead of the body
% of the paper. For a more streamlined reading experience, I have placed all the
% details here.} 
% \subsubsection{Dataset generation}
\ej{Some of this is likely to change as I iterate on datasets.}
To have ground truth statistical models, we simulated both datasets. We started
from causal models based on those presented in research papers about
income~\ej{\cite{}} and education~\ej{\cite{}}. When simulating the datasets, we
ensured the causal models and variables exhibited properties (e.g., confounding,
categorical data types) where common modeling mistakes would lead to incorrect
statistical models and results. 

We identified the following modeling mistakes from textbooks
(McElreath~\cite{mcelreath2020statistical} Gelman and
Hill~\cite{gelmanHill2006regression}; and Cohen, Cohen, West, and
Aiken~\cite{cohen1988statistical}) and recent statistical
research~\cite{barr2013random,barr2013randomUpdated} that we anticipated
participants to make: 
\begin{enumerate}
    \item Omitting an important \diff{fixed} variable that would change the magnitude and statistical significance of coefficients of all other variables
    \item Multicollinearity: Including unnecessary \diff{fixed} variables that change the magnitude and statistical significance of all other variables [not sure how to simulate this yet]
    \item Omitting an interaction (\ej{within/across/both levels?}) that would change the magnitude and statistical significance of all other coefficients
    \item Assuming Gaussian/identity link (linear regresion) inappropriately
    \item Using a log transform leads to different results as when using a log link function [not sure how to siumlate this yet]
    \item \diff{Excluding random effects}
    \item \diff{Specifying sub-maximal random effects}
    \item \diff{Including unidentifiable random effects}
\end{enumerate} 

We developed \ej{Q} analysis questions (1 per mistake) intentionally designed to lead
participants to erroneous models without careful consideration. We included an
open-ended analysis question that was always at the very end to contrast how
participants may analyze the dataset more freely.

\ej{Include the causal models, analysis questions, answers to the questions as supplementary material.}

\subsection{Measures}
\textit{Error:} For each analysis question, we first determined if the
participant discovered the ground truth model (binary outcome). If not, we
quantified the severity of the error as the difference in \textbf{model fit}
(i.e., AIC, BIC, Adjusted R-squared), the \textbf{coefficients} for each
variable (i.e., the signs of coefficients and the absolute values/relative
magnitudes of coefficients), and the \textbf{uncertainty} associated with each
variable (i.e., standard errors, confidence intervals, and p-values).

In a qualitative analysis, we (i) identified the observable error (e.g., exclude a key
variable) in the submitted model and (ii) conducted a root cause analysis from
the recorded audio and video traces. We looked for the chain of assumptions and
decisions that led to the error. To identify common sources of error, we
compared the chains of actions leading to observed errors across participants.

\ej{Should the root cause analysis be conducted with the participant at the end lab study or in a follow-up session? Rather than among the researchers afterwards?}

% The researcher also asked follow-up questions
% in the closing interview to probe into the analysts' rationale for each observed
% error. 

\textit{Learning:} We thematically analyzed participants' responses to the
post-survey and semi-structured interview questions about what they learned
about their data and analytical approaches from their experience using Tisane.

\ej{Should we ask about what they learned from their analyses without Tisane?}

\subsection{Findings}
\ej{TBD!}

\subsection{Discussion}
\ej{Update this once I have read up on related work on error classification systems...}
For errors, we should relate the observed chains and observed errors to Norman's
model of error (slips vs. mistakes); Rasmussen's modes of behavior (skill vs.
rule vs. knowledge); hypothesis formalization (?).


\section{Study 3: Evaluating the impact of Tisane on authoring GLMMs for non-nesting composition}
Best practices recommend analysts use maximal mixed-effects models in settings
with non-nesting composition~\cite{barr2013random,barr2013randomUpdated}. We
chose to study the impact of Tisane on analyses involving non-nesting
compositions separately from settings with hierarchical data and repeated
measures because we did not find examples of study designs or datasets in
textbooks that exhibited all three data measurement relationships simultaneously. 
\ej{Ideally, I think we would be able to simulate a dataset with all three settings that require random effects (hierarchical data, repeated measures, and non-nesting composition). I can think more about a dataset that could exhibit all three, but this seems uncommon.}

The methods are identical to Study 2 except that the datasets will contain
non-nesting compositions but no data hierarchies or repeated measures. My
current plan is to generate datasets similar to the lexical decision task Barr
et al. use to make the case for maximal random effects~\cite{barr2013random}.

==> archive/hypotheses.tex <==
\section{Hypotheses}
\begin{itemize}
    \item When using Tisane, participants will make fewer mistakes in selecting and specifying
    statistical models than when they use...
    \item After using Tisane, participants will report an increased awareness of
    their data, conceptual assumptions, and possible statistical models. 
    \item \ej{Should add something more general about statistical education?}
\end{itemize}


==> archive/protocol_graphs.tex <==
\newcommand{\SchoolIncomeGraph}{
    \begin{figure}[H]
        \def\arrowend{.4}
        \def\dotsbegin{.43}
        \def\dotsend{.55}
        \def\arrowbegin{.59}
        \begin{tikzpicture}
            \node[fill=gray!10,rounded corners=4pt]	(n3)	{%
                \begin{tikzpicture}[>=Stealth,
                                    causes/.style={draw=black},
                                    measure/.style={fill=white,min,circle,draw=black},
                                    depvar/.style={fill=gray!30},
                                    every edge quotes/.style={fill=none,fill opacity=.9,text opacity=1,rounded corners=3pt,inner sep=2pt,node font=\scriptsize},
                                    tightly/.style={inner sep=1pt},
                                    loosely/.style={inner sep=.7em},
                                    scale=0.9,transform shape]
                    \node[measure]	(edu)		{Education};
                    % \node[measure,left=of edu]	(income)		{\footnotesize CME};
                    % \node[measure,right=of iv]	(m2)		{\footnotesize CME};
                    \node[measure,depvar, below=of edu]	(income)		{Income};
                    % \node[measure,depvar,above=of iv]	(dv)	{DV};

                    \graph{
                        (edu) -> [causes, "  ???", below, right] (income);
                        % (iv) ->[associates,below] (m2);
                        % (iv) ->[associates,left] (m3);
                        % % (m1) ->[associates,below] (iv);
                        % (m2) ->[associates,above] (iv);
                        % (m3) ->[associates,right] (iv);
                        % (dv) ->[associates,below right] (m1);
                        % (m1) ->[associates,above left] (dv);
                        % % (dv) ->[draw=black,"assoc.",below right,pos=0.25] (m1);
                        % % (m1) ->[associates,bend left,above left] (dv);
                        % (m2) ->[associates,above right] (dv);
                        % (dv) ->[draw=black,"assoc.",below left,pos=0.25] (m2);
                    };
                \end{tikzpicture}
            };

        \end{tikzpicture}
        \caption{Single cause}
        % \label{fig:figureOnlyAssociatesOrCausesEdgesCandidateMainEffects}
    \end{figure}
}

\newcommand{\SchoolSexIncomeGraph}{
    \begin{figure}[H]
        \def\arrowend{.4}
        \def\dotsbegin{.43}
        \def\dotsend{.55}
        \def\arrowbegin{.59}
        \begin{tikzpicture}
            \node[fill=gray!10,rounded corners=4pt]	(n3)	{%
                \begin{tikzpicture}[>=Stealth,
                                    causes/.style={draw=black},
                                    measure/.style={fill=white,min,circle,draw=black},
                                    depvar/.style={fill=gray!30},
                                    every edge quotes/.style={fill=none,fill opacity=.9,text opacity=1,rounded corners=3pt,inner sep=2pt,node font=\scriptsize},
                                    tightly/.style={inner sep=1pt},
                                    loosely/.style={inner sep=.7em},
                                    scale=0.9,transform shape]
                    \node[measure]	(edu)		{Education};
                    \node[measure, left=of edu]	(sex)		{Sex};
                    \node[measure,depvar, below=of edu]	(income)		{Income};
                    \graph{
                        (edu) -> [causes, "  ???", below, right] (income);
                        (sex) -> [causes, below] (income);
                        (sex) -> [causes, right] (edu);
                    };
                \end{tikzpicture}
            };

        \end{tikzpicture}
        \caption{DAG structure: Fork}
        % \label{fig:figureOnlyAssociatesOrCausesEdgesCandidateMainEffects}
    \end{figure}
}

\newcommand{\SchoolOccupationIncomeGraph}{
    \begin{figure}[H]
        \def\arrowend{.4}
        \def\dotsbegin{.43}
        \def\dotsend{.55}
        \def\arrowbegin{.59}
        \begin{tikzpicture}
            \node[fill=gray!10,rounded corners=4pt]	(n3)	{%
                \begin{tikzpicture}[>=Stealth,
                                    causes/.style={draw=black},
                                    measure/.style={fill=white,min,circle,draw=black},
                                    depvar/.style={fill=gray!30},
                                    every edge quotes/.style={fill=none,fill opacity=.9,text opacity=1,rounded corners=3pt,inner sep=2pt,node font=\scriptsize},
                                    tightly/.style={inner sep=1pt},
                                    loosely/.style={inner sep=.7em},
                                    scale=0.9,transform shape]
                    \node[measure] (edu) {Education};
                    \node[measure,depvar, below=of edu]	(income)		{Income};
                    \node[measure, left=of income] (occ) {Occupation};
                    \graph{
                        (edu) -> [causes, below] (income);    
                        (edu) -> [causes, "  ???", below, left] (occ);    
                        (occ) -> [causes, right] (income);
                        
                    };
                \end{tikzpicture}
            };

        \end{tikzpicture}
        \caption{DAG structure: Collider}
        % \label{fig:figureOnlyAssociatesOrCausesEdgesCandidateMainEffects}
    \end{figure}
}

\newcommand{\RaceSchoolIncomeGraph}{
    \begin{figure}[H]
        \def\arrowend{.4}
        \def\dotsbegin{.43}
        \def\dotsend{.55}
        \def\arrowbegin{.59}
        \begin{tikzpicture}
            \node[fill=gray!10,rounded corners=4pt]	(n3)	{%
                \begin{tikzpicture}[>=Stealth,
                                    causes/.style={draw=black},
                                    measure/.style={fill=white,min,circle,draw=black},
                                    depvar/.style={fill=gray!30},
                                    every edge quotes/.style={fill=none,fill opacity=.9,text opacity=1,rounded corners=3pt,inner sep=2pt,node font=\scriptsize},
                                    tightly/.style={inner sep=1pt},
                                    loosely/.style={inner sep=.7em},
                                    scale=0.9,transform shape]
                    \node[measure]	(edu)		{Education};
                    \node[measure, above=of edu]	(race)		{Race};
                    \node[measure,depvar, below=of edu]	(income)		{Income};
                    \graph{
                        (race) -> [causes, below] (edu);
                        (edu) -> [causes, below] (income);
                        (race) -> [causes, " ???", below, right, bend left=50] (income);
                    };
                \end{tikzpicture}
            };

        \end{tikzpicture}
        \caption{DAG structure: Pipe}
        % \label{fig:figureOnlyAssociatesOrCausesEdgesCandidateMainEffects}
    \end{figure}
}

\newcommand{\AgeRaceSchoolIncomeGraph}{
    \begin{figure}[H]
        \def\arrowend{.4}
        \def\dotsbegin{.43}
        \def\dotsend{.55}
        \def\arrowbegin{.59}
        \begin{tikzpicture}
            \node[fill=gray!10,rounded corners=4pt]	(n3)	{%
                \begin{tikzpicture}[>=Stealth,
                                    causes/.style={draw=black},
                                    measure/.style={fill=white,min,circle,draw=black},
                                    depvar/.style={fill=gray!30},
                                    every edge quotes/.style={fill=none,fill opacity=.9,text opacity=1,rounded corners=3pt,inner sep=2pt,node font=\scriptsize},
                                    tightly/.style={inner sep=1pt},
                                    loosely/.style={inner sep=.7em},
                                    scale=0.9,transform shape]
                    
                    % \node[measure] (edu) at ($(age)!0.5!(race)$) {Education};
                    \node[measure] (edu) {Education};
                    \node[measure, right=of edu]	(age)		{Age};
                    \node[measure, above=of edu]	(race)		{Race};
                    \node[measure,depvar, below=of edu]	(income)		{Income};
                    % \node[measure, left=of income] (occ) {Occupation};
                    \graph{
                        (edu) -> [causes, below] (income);    
                        (age) -> [causes, left] (edu);
                        (race) -> [causes, below] (edu);
                        (age) -> [causes, " ???", below, right] (income);
                    };
                \end{tikzpicture}
            };

        \end{tikzpicture}
        \caption{DAG structure: Descendant}
        % \label{fig:figureOnlyAssociatesOrCausesEdgesCandidateMainEffects}
    \end{figure}
}

\newcommand{\CompleteIncomeGraph}{
    \begin{figure}[H]
        \def\arrowend{.4}
        \def\dotsbegin{.43}
        \def\dotsend{.55}
        \def\arrowbegin{.59}
        \begin{tikzpicture}
            \node[fill=gray!10,rounded corners=4pt]	(n3)	{%
                \begin{tikzpicture}[>=Stealth,
                                    causes/.style={draw=black},
                                    measure/.style={fill=white,min,circle,draw=black},
                                    depvar/.style={fill=gray!30},
                                    every edge quotes/.style={fill=none,fill opacity=.9,text opacity=1,rounded corners=3pt,inner sep=2pt,node font=\scriptsize},
                                    tightly/.style={inner sep=1pt},
                                    loosely/.style={inner sep=.7em},
                                    scale=0.9,transform shape]
                    
                    % \node[measure] (edu) at ($(age)!0.5!(race)$) {Education};
                    \node[measure] (edu) {Education};
                    \node[measure, right=of edu]	(age)		{Age};
                    \node[measure, above=of edu]	(race)		{Race};
                    \node[measure, left=of edu]	(sex)		{Sex};
                    \node[measure,depvar, below=of edu]	(income)		{Income};
                    \node[measure, left=of income] (occ) {Occupation};
                    \graph{
                        (edu) -> [causes, below] (income);    
                        (sex) -> [causes, right] (edu);
                        (sex) -> [causes, below] (income);
                        (occ) -> [causes, right] (income);
                        (age) -> [causes, left] (edu);
                        (race) -> [causes, below] (edu);
                        
                    };
                \end{tikzpicture}
            };

        \end{tikzpicture}
        \caption{Complete DAG that contains all four structures: fork, collider, pipe, and descendant}
        % \label{fig:figureOnlyAssociatesOrCausesEdgesCandidateMainEffects}
    \end{figure}
}


% \SchoolIncomeGraph
% \SchoolSexIncomeGraph
% \SchoolOccupationIncomeGraph
% \RaceSchoolIncomeGraph
% \AgeRaceSchoolIncomeGraph
% \CompleteIncomeGraph





\newcommand{\HealthDentalTimeGraph}{
    \begin{figure}[H]
        \def\arrowend{.4}
        \def\dotsbegin{.43}
        \def\dotsend{.55}
        \def\arrowbegin{.59}
        \begin{tikzpicture}
            \node[fill=gray!10,rounded corners=4pt]	(n3)	{%
                \begin{tikzpicture}[>=Stealth,
                                    causes/.style={draw=black},
                                    measure/.style={fill=white,min,circle,draw=black},
                                    depvar/.style={fill=gray!30},
                                    every edge quotes/.style={fill=none,fill opacity=.9,text opacity=1,rounded corners=3pt,inner sep=2pt,node font=\scriptsize},
                                    tightly/.style={inner sep=1pt},
                                    loosely/.style={inner sep=.7em},
                                    scale=0.9,transform shape]
                    \node[measure]	(genHealth)		{Health};
                    \node[measure,depvar, below=of genHealth]	(time)		{Time};
                    \graph{
                        (genHealth) -> [causes, " ???", below, right] (time);

                        % % (dv) ->[draw=black,"assoc.",below right,pos=0.25] (m1);
                    };
                \end{tikzpicture}
            };

        \end{tikzpicture}
        \caption{Single cause}
    \end{figure}
}

\newcommand{\RegionHealthTimeGraph}{
    \begin{figure}[H]
        \def\arrowend{.4}
        \def\dotsbegin{.43}
        \def\dotsend{.55}
        \def\arrowbegin{.59}
        \begin{tikzpicture}
            \node[fill=gray!10,rounded corners=4pt]	(n3)	{%
                \begin{tikzpicture}[>=Stealth,
                                    causes/.style={draw=black},
                                    measure/.style={fill=white,min,circle,draw=black},
                                    depvar/.style={fill=gray!30},
                                    every edge quotes/.style={fill=none,fill opacity=.9,text opacity=1,rounded corners=3pt,inner sep=2pt,node font=\scriptsize},
                                    tightly/.style={inner sep=1pt},
                                    loosely/.style={inner sep=.7em},
                                    scale=0.9,transform shape]
                                    \node[measure]	(genHealth)		{Health};
                                    \node[measure, left=of genHealth]	(region)		{Region};
                                    \node[measure,depvar, below=of genHealth]	(time)		{Time};
                    \graph{
                        (genHealth) -> [causes, " ???", below, right] (time);
                        (region) -> [causes, below] (time);
                        (region) -> [causes, right] (genHealth);
                    };
                \end{tikzpicture}
            };

        \end{tikzpicture}
        \caption{DAG structure: Fork}
        % \label{fig:figureOnlyAssociatesOrCausesEdgesCandidateMainEffects}
    \end{figure}
}

\newcommand{\HealthCountyTimeGraph}{
    \begin{figure}[H]
        \def\arrowend{.4}
        \def\dotsbegin{.43}
        \def\dotsend{.55}
        \def\arrowbegin{.59}
        \begin{tikzpicture}
            \node[fill=gray!10,rounded corners=4pt]	(n3)	{%
                \begin{tikzpicture}[>=Stealth,
                                    causes/.style={draw=black},
                                    measure/.style={fill=white,min,circle,draw=black},
                                    depvar/.style={fill=gray!30},
                                    every edge quotes/.style={fill=none,fill opacity=.9,text opacity=1,rounded corners=3pt,inner sep=2pt,node font=\scriptsize},
                                    tightly/.style={inner sep=1pt},
                                    loosely/.style={inner sep=.7em},
                                    scale=0.9,transform shape]
                                    \node[measure]	(genHealth)		{Health};
                                    \node[measure,depvar, below=of genHealth]	(time)		{Time};
                                    \node[measure, left=of time] (county) {County};
                    \graph{
                        (genHealth) -> [causes, below] (time);    
                        (county) -> [causes, right] (time);
                        (genHealth) -> [causes, " ???", below, left] (county);
                    };
                \end{tikzpicture}
            };

        \end{tikzpicture}
        \caption{DAG structure: Collider}
        % \label{fig:figureOnlyAssociatesOrCausesEdgesCandidateMainEffects}
    \end{figure}
}

\newcommand{\InsuranceHealthTimeGraph}{
    \begin{figure}[H]
        \def\arrowend{.4}
        \def\dotsbegin{.43}
        \def\dotsend{.55}
        \def\arrowbegin{.59}
        \begin{tikzpicture}
            \node[fill=gray!10,rounded corners=4pt]	(n3)	{%
                \begin{tikzpicture}[>=Stealth,
                                    causes/.style={draw=black},
                                    measure/.style={fill=white,min,circle,draw=black},
                                    depvar/.style={fill=gray!30},
                                    every edge quotes/.style={fill=none,fill opacity=.9,text opacity=1,rounded corners=3pt,inner sep=2pt,node font=\scriptsize},
                                    tightly/.style={inner sep=1pt},
                                    loosely/.style={inner sep=.7em},
                                    scale=0.9,transform shape]
                                    \node[measure]	(genHealth)		{Health};
                                    \node[measure,depvar, below=of genHealth]	(time)		{Time};
                                    \node[measure, above=of genHealth]	(insurance)		{Insurance};
                    \graph{
                        (insurance) -> [causes, below] (genHealth);
                        (genHealth) -> [causes, below] (time);
                        (insurance) -> [causes, " ???", below, right, bend left=50] (time);
                    };
                \end{tikzpicture}
            };

        \end{tikzpicture}
        \caption{DAG structure: Pipe}
        % \label{fig:figureOnlyAssociatesOrCausesEdgesCandidateMainEffects}
    \end{figure}
}

\newcommand{\WorkInsuranceHealthTimeGraph}{
    \begin{figure}[H]
        \def\arrowend{.4}
        \def\dotsbegin{.43}
        \def\dotsend{.55}
        \def\arrowbegin{.59}
        \begin{tikzpicture}
            \node[fill=gray!10,rounded corners=4pt]	(n3)	{%
                \begin{tikzpicture}[>=Stealth,
                                    causes/.style={draw=black},
                                    measure/.style={fill=white,min,circle,draw=black},
                                    depvar/.style={fill=gray!30},
                                    every edge quotes/.style={fill=none,fill opacity=.9,text opacity=1,rounded corners=3pt,inner sep=2pt,node font=\scriptsize},
                                    tightly/.style={inner sep=1pt},
                                    loosely/.style={inner sep=.7em},
                                    scale=0.9,transform shape]
                    
                    % \node[measure] (edu) at ($(age)!0.5!(race)$) {Education};
                    \node[measure]	(genHealth)		{Health};
                    \node[measure,depvar, below=of genHealth]	(time)		{Time};
                    \node[measure, above=of genHealth]	(insurance)		{Insurance};
                    \node[measure, right=of genHealth]	(hours)		{Work hours};
                    % \node[measure, left=of income] (occ) {Occupation};
                    \graph{
                        (insurance) -> [causes, below] (genHealth);
                        (hours) -> [causes, left] (genHealth);
                        (genHealth) -> [causes, below] (time);
                        (hours) -> [causes, "  ???", below, right] (time);
                    };
                \end{tikzpicture}
            };

        \end{tikzpicture}
        \caption{DAG structure: Descendant}
        % \label{fig:figureOnlyAssociatesOrCausesEdgesCandidateMainEffects}
    \end{figure}
}

==> archive/qual_lab_study.tex <==
\def\unit{\texttt{Unit}\xspace}
\def\measure{\texttt{Measure}\xspace}
\def\setup{\texttt{SetUp}\xspace}

\section{Exploratory study}
% Motivation
% Our motivating question was, ``What implicit semantics do analysts use to construct conceptual models of how variables relate?''. 
Our primary aim was to uncover how analysts internally represent knowledge about
a research topic and a study design necessary for statistical modeling. We
probed analysts' internal processes by prompting them to use an existing
domain-specific language for eliciting and expressing conceptual models and
study designs in service of authoring statistical models. Based on the answers
to our research questions, we derived design implications
(\autoref{sec:design_implications}) that informed the design of \tisane.

\subsection{Method}
%Participants
We conducted a lab study with five computer science PhD students who were
enrolled in a quantitative research methods course. We recruited participants
through the course as a convenience sample so that we could control their recent
exposure to statistical concepts. All participants self-reported that they
conducted research in programming languages or software engineering and planned
to perform statistical analyses in future research projects. 
% \ej{Add: Approaches, mindsets of participants as they were completing the study}

The study consisted of two parts: (i) a take-home assignment and (ii) an in-lab
session. The take-home assignment asked participants to read a recently
published CHI paper~\cite{winters2021heartbeat}, identify the research questions
and hypotheses, describe the authors' conceptual models, summarize the study
design, and consider alternative ways of analyzing the data to answer the
research questions. The assignment was designed to ensure that participants
engaged with the paper's key ideas prior to the lab study. We chose the specific
paper because we believed its topic (i.e., empathetic biosignals) would be
broadly approachable and the statistical methods used (i.e., generalized linear
models) would be familiar with students enrolled in the research methods course.
% On a scale from
% one (not at all relatable) to five
% (extremely relatable), four participants indicated that the paper was relatable
% with a score of 3 or higher.

After submitting the homework, participants were elligible to participate in the
lab session. The lab session followed a semi-structured, think-a-loud protocol.
The researcher reviewed each submission to prepare participant-specific
questions. The lab study used Tisane~\cite{jun2022tisane}, an open-source
package for authoring generalized linear models with or without mixed effects,
as a probe to understand how participants thought about and wanted to express
their conceptual models and study designs. We adapted Tisane's Python API into R
syntax for the study since the research methods course taught and used R. We
used Tisane because of its focus on eliciting both conceptual model and study
designs in one system from end-users. Using Tisane simplified the study protocol
compared to using separate tools for conceptual models and study design. 

Upon entering the lab, participants reviewed their homework submission to remind
themselves of the paper, which was referenced and available throughout the lab
study. Participants also had a hardcopy of the paper they could refer back to at
any time on the lab desk next to them. Then, participants engaged in three task:
expressing (i) variable proxies, (ii) conceptual models, and (iii) study
designs. For each task, participants started with Tisane's language constructs
to express their intent and discussed their confusions, how they understood each
presented construct, and what they wanted to say but could not (if applicable).
The researcher repeatedly reminded participants that the constructs presented
were prototype possibilities and that expressing their intentions was more
important than using the constructs or getting the syntax correct. Throughout,
the researcher paid particular attention to where Tisane broke down for
participants and asked follow-up questions to probe deeper into why. The
researcher considered such breakdowns as openings into semantic mismatches
between the end-user and the system. 

% Analysis 
We iteratively coded homework submissions, audio transcripts from the lab study
sessions, and lab study artifacts to uncover our findings. We also consulted the
researcher's detailed notes from the lab sessions. 

% Based on an iteraWe conducted a content analysis of the produced code suggestions (output
% artifacts) along with a thematic analysis of the audio transcripts from each lab
% session. 

\subsection{Key Observations and Design Implications}
All participants demonstrated a working knowledge of the assigned paper's
motivating research questions, study design, and general study procedure. 
% Among
% the submitted conceptual models, four were a list of conceptual relationships,
% and one was a diagram. 
We made two key observations about what and how statistical non-experts wanted
to express their conceptual models. Below, we elaborate on these observations
and derive design implications for systems that connect conceptual and
statistical modeling, which we implement in \rTisane (see~\autoref{sec:system}).

\subsubsection{Participants want to express conceptual knowledge at varying degrees of specificity.}
Contrary to the popular belief that higher levels of abstraction are better for
domain or programming novices, we found that statistical non-experts want to
move up and down the ladder of abstraction when expressing conceptual models. 

When defining ``causes,'' P2 described ``[Causes] is...like when we teach
logic...it's like implication, right?....So I'm saying if we are observing an
emotion and...emotion observed can lead to a change in emotional perspective.''
P0, P1, and P3 contrasted a bidirectional relationship between variables,
formerly encapsulated in the \texttt{associates\_with} construct in \tisane, to
their implicit understanding of ``causes.'' For instance, P1 stated ``the most
like, utilitarian definition by if A causes B, then by changing A, I can change
B whereas \texttt{associates\_with} means that...if I can turn dial A, B might
not change.'' In addition to differentiating between causal and associative
relationships, three participants [P0, P1, P3] provided statements of
\textit{specifically how} a variable influenced another in the conceptual models
submitted as homework. For example, P0 wrote, ``Hearing a heartbeat that seems to
be aligned with visual cues makes someone feel \textit{more} strongly what
another person is feeling'' (emphasis added), specifying a (positive)
directionality to the influence from ``hearting a heartbeat'' to empathy. 

These observations suggest that analysts have an intuitive understanding of
causality but stating that a variable causes another is insufficient to capture
the richness of their conceptual models. \textbf{Analysts want to be able to
describe how a variable influences another.}
\paragraph{Design implication: Allow analysts to express *how* xvariables influence one another --> when then}

%   in addition to vaguer statements without a clear
% positive/negative direction, such as ``Visual cues directly influence a person’s
% perception of another’s emotions'' [P0]. 
% The homework assignment and lab study materials may have primed participants to
% think about ``direct'' and ``indirect'' relationships and commutativity, so
% analysts' descriptions of causal relationships as ``unidirectional'' and
% associative relationships as ``bidirectional'' were not surprising [P0, P2, P3].

% how a bidirectional relationship between two variables 
% indicative of proxies measuring the same latent construct (``...for two things
% to be bi-directional and for it to be a really, really direct relationship. Like
% that just never happens in the real world without them turning out to be like
% proxies for the same exact thing.'') [P3]; and that 

Furthermore, participants consistently found Tisane's \texttt{moderates}
construct difficult to understand [P0, P1, P2, P3]. Although designed for
specifying interaction variables, participants found the \texttt{moderates}
construct could be overloaded....START HEREntroduced
confusion between what it implied in terms of how two variables were related
conceptually. 
what the term meant: ``I'm not really sure of the `moderates.' I'm not super
familiar with that term.'' Thus, she interpreted the definition of `moderates'
as ``just like multiple things that may cause or associate.'' P4 did not express
frustration or confusion with the construct but misunderstood it as a synonym
for ``associates with'' since both constructs were commutative. P3, who
demonstrated a familiarity with the term and concept of moderation, grappled
with if ``moderates'' was shorthand for expressing associative relationships
between each independent variable and the dependent variable, how moderation
implies causal relationships, and if statistical and conceptual definitions of
moderation differed from each other: ``[L]et's say there's two independent
variables and one dependent variable. And each of the [independent] variables
individually is not correlated with the outcome. But if you put them together,
then the correlation appears....I mean, it's sort of a philosophical question of
whether, like each of the ones individually causes [the dependent variable] in
that case. But thinking from a...statistical perspective, I think that's a
situation where you might be able to express...language and experience level
together cause lines of code but individually they don't because no individual
correlation would appear there.'' These observations suggest that (i) the
semantics of moderation is unclear in Tisane and (ii) moderation may be easier
to reason about when decomposed into what happens to the dependent variable when
two or more independent variables have specific values. 
\paragraph{Design implication: Too high level --> Remove moderates}

In addition to detailing how variables influence one another, participants also grappled
with what specific structures in a conceptual model meant. P1 and P3 described
how a bidirectional relationship between two variables were really due to
hidden, confounding variables causing both variables. P3 described how ``in the
real world, when, when these bidirectional things happen, it means there's sort
of this middleman complex system. Or some like underlying process of which [two
variables are] both components...'' Another participant, P2, wondered aloud
about how even what appears like a direct relationship, may actually be a chain
of indirect or mediated relationships at a lower granularity: ``It's like Google
Maps. If you zoom out enough, that arrow becomes a direct arrow.'' These
observations suggest that while participants can deeply reflect on what could be
happening between variables conceptually, \textbf{they need help exploring and
figuring out which of these structures to use in their data analyses.}
% P3's definition of associative relationships
% is consistent with an associative structure called a ``fork'' in causal DAGs.
\paragraph{Need help exploring and picking among possible structures.}

Participants also \textit{distinguished between known and suspected
relationships} [P0, P1, P2, P3, P4]. Participants described known relationships
established in prior work as ``assupmtions'' or ``assertions'' to check
separately from the key research questions that ``tested'' suspected
relationships. P0 described how ``maybe we have to differentiate as to like the
known [relationships] are kind of the things you're \textit{assuming} there's
relationships between these things whereas the suspected...[are] the things kind
of like your research questions are saying like, `We think there's this
relationship but...it's what we're testing for.'' (emphasis added). Similarly,
P4 suggested that Tisane should warn end-users when assumptions about known
relationships are violated in a given data set: ``I would also say that it would
be very handy to be able to say, kind of \textit{assert} that language has no
effect on the line of code. And be warned if it's not the case, like if your
\textit{assertion} is not...verified automatically with the DSL, but
warned...that while your \textit{assumption} is not holding there is actually an
effect, which could be very handy on your study.'' (emphasis added). However,
Tisane does not differentiate between known and suspected relationships, and as
P4 noted, ``I don't know if everything that is not either specified to moderate,
associate, or causes is by default, asserting that there is no effect,''
suggesting that the Tisane's DSL semantics could be more self-evident. 
In fact, one of the reasons that analysts repeatedly expressed preferring less
technical verbs, such as
``influences'' [P0] or ``leads to'' [P3], may be due to the inability to
indicate relationships that are known vs. suspected in \tisane. For instance, P0
explained how she preferred ``influences'' over ``causes'' because ``I guess
it's like \textit{a level of sureness} in it in which, like, `cause' feels more confident
in your answers than `influences''' (emphasis added).
\paragraph{Design implication: Provide constructs for distinguishing betwen known and suspected relationships -->  assume/hypothesize}


\subsubsection{More expressivity for specifying study designs/experimental design}
**keep short**
Additional observations about expressing study design
More future work for how to express study designs

\paragraph{Participant construct - syntactic sugar for Unit}

\paragraph{Condition construct - syntactic sugar?}

Moreover, analysts expected \textit{experimental conditions to be standalone
concepts}. In Tisane, experimental conditions can be specified as a \measure of
a \unit. Instead, P0 and P4 had separate conceptual categories for conditions
and measures in their mental models of study designs. P4 preferred a separate
condition data type currently unavailable in Tisane because the term ``Measure''
did not create a ``bucket'' appropriate for conditions. P4 resorted to declaring
condition as a \setup variable, violating the intended semantics of \setup
variables in Tisane: ``Like it doesn't feel like the condition are measured.
Right? I'm measuring the proxy. I'm not measuring the condition. So to me,
that's why I'm putting the visual on the four condition as a...\setup
variable.'' Similar to P4, when P0 saw the ``SetUp'' class, she thought it
described conditions: ``[I]f I heard the word `setup,' I would think of more
like conditions like, like, this person uses this IDE or this person is given
this IDE.'' 

Participants were also interested in \textit{representing trials (and stimuli)
and responses elicited during each trial explicitly}. All participants discussed
wanting to explicitly represent trials alongside participants as a \unit or a
\setup variable, which may not match Tisane DSL's structuring of data
measurement relationships: ``I want to have a trial unit that is nested within
trials, which is nested within or maybe I could just have trial nested within
Participant, but I'm not seeing a way to clearly delineate or like to denote
that'' [P1]. In Tisane, nesting a trial within a participant would mean that
multiple trials exist in each participant (e.g., akin to how multiple children
exist in a family), which even in natural language, does not capture what P1
wanted to convey, which was that each participant sees and provides responses
for each trial. 

\subsection{Discussion: Design Implications} \label{sec:design_implications} 

Our observations about how participants internally represent conceptual models
and study designs have two implications for improving the design of Tisane.

\textbf{Deconstruct statistical constructs for clarity.}
Unsurprisingly, we found that class and function names such as ``Measure,''
``SetUp,'' and ``moderates'' confused participants. These names either suggested
informal conceptual categories or were too close to statistical jargon. As a
result, connecting a Tisane program's semantics to a mental model of study
design was challenging. Particularly insightful was participants' consternation
with the function ``moderates.'' Participants could reason about the details of
moderation relationships but did not know what the term meant or how to use it
to clearly communicate their conceptual models in detail. Using
specific,granular language constructs (e.g., pairwise relationships) and
allowing for system-gudiance to consider more complex statistical structures
(e.g., interaction effects for moderation) may help analysts more accurately
understand and use Tisane.

\textbf{Allow for conceptual ambiguity, make specificity optional.}
Despite being statistical non-experts, participants were noticeably focused on
low-level details about conceptual relationships. All participants
differentiated between known and suspected relationships and generally agreed
that known relationships should be checked for prior to assessing the suspected,
or ambiguous, ones. At the same time, when participants were confident about
some relationships, they were specific about if the relationships were
positive/negative. Welcoming ambiguity and specificity could help analysts write
and use conceptual models throughout data analysis and interpretation.

Both design implications suggest the need to re-structure Tisane's programming
and interaction models. First, Tisane's specification language needs to be more
specific and low-level. This finding is \textit{counterintuitive} because a
well-documented strategy for making programming tasks easier for non-experts has
been to raise the level of abstraction for a programming
domain~\cite{chasins2018rousillon,satyanarayan2017vega}. Yet, we have evidence
that suggests the opposite for specifying a conceptual model and study design.
Second, Tisane's specification process could be more tiered, and disambiguation
could leverage ambiguity in analysts' specification as opportunities for more
numerous intelligent suggestions and guidance. 

\todo{Mention that the focus needs to be on conceptual level, but within conceptual level, there should be opportunity to move up and down the ladder of conceptual abstraction}

%hand-offs to a reasoning engine to suggest possible analysis paths, for example. 

% the conceptual modeling and study design specification process to be more tiered

==> archive/study.tex <==
%%% Income dataset
\SchoolIncomeGraph
\SchoolSexIncomeGraph
\SchoolOccupationIncomeGraph
\RaceSchoolIncomeGraph
\AgeRaceSchoolIncomeGraph

%%% Dental health dataset
\HealthDentalTimeGraph

\RegionHealthTimeGraph

\HealthCountyTimeGraph

\InsuranceHealthTimeGraph

\WorkInsuranceHealthTimeGraph

==> archive/summative_eval.tex <==
\section{Summative Evaluation}
We had three research questions:

\begin{itemize}
    \item \evalConceptualModels What is the influence of rTisane on conceptual
    modeling?
    \item \evalStatisticalModels How does rTisane impact the statistical models
    analysts implement? Specifically, do the covariates, family functions, and
    link functions analysts include/exclude differ when implementing statistical
    models on their own vs. using rTisane? How well do statistical models
    analysts author on their own vs. using rTisane fit the data?  
    \item \evalLearning Do analysts learn about their discipline or data
    analysis as a result of using rTisane?
\end{itemize}

\subsection{Study design}
% \todo{Include a diagram summarizing study design?}
We conducted a within-subjects think-a-loud lab study that consisted of four phases: 

\begin{itemize}
    \item \textbf{Phase 1: Warm up.} We presented participants with the
    following open-ended research question: ``What aspects of an adult’s
    background and demographics are associated with income?'' We asked
    participants to specify a conceptual model including variables they thought
    influenced income. This warm-up exercise helped to externalize and keep
    track of participants' pre-conceived notions and assumptions prior to seeing
    a more restricted data schema.
    \item \textbf{Phase 2: Express conceptual models} We presented participants
    with a data schema describing a dataset from the U.S. Census Bureau. We then
    asked participants to specify a conceptual model using only the available
    variables. At the end, we asked participants about their
    experiences specifying their conceptual models in a brief survey and semi-structured interview.
    \item \textbf{Phase 3: Implement statistical models} We asked participants
    to implement ``a statistical model that assesses the influence of variables
    [they] believe to be important (in the context of additional potentially
    influential factors) on income,'' relying on only their conceptual model. We
    then asked participants about their experiences implementing statistical
    models through a brief survey and semi-structured interview. 
    \item \textbf{Phase 4: Exit interview.} The study concluded with a survey
    and semi-structured interview where we asked participants to reflect on the
    process of explicitly connecting conceptual models to statistical models.
\end{itemize} 

We designed the study based on the assumption that conceptual modeling is a
helpful strategy when specifying statistical models. As a result, all
participants completed the phases in the above order. In order to assess the
effect of tooling on conceptual models and the quality of statistical models, we
counterbalanced the order in which participants specified conceptual and
statistical models. Half the participants specified their conceptual and
statistical models on their own (without rTisane) first. The other started with
rTisane.

\noindent \paragraph{Participants} We recruited \ej{24?} data analysts on
Upwork. We screened for participants who reported having experience with
authoring generalized linear models and using R. \ej{On average, participants
reported having conducted N projects using generalized linear models.
Participants were familiar with a range of software tools, including...} All
studies were conducted over Zoom. Each participant was compensated \ej{\$50} for
120 minutes of their time. We recorded participants' screens, video, and audio
throughout the study. We then transcribed the audio for qualitative analyses.

% One dataset was on demographic factors and income in the U.S. in 2018 from the
% U.S. Census Bureau (\datasetIncome). The other dataset was about demographic
% factors and health conditions in the U.S. (\datasetHealth) from \ej{FILL IN}.
% More information on how the datasets were created are found in the
% supplemental material.

\subsection{Analysis and Results}
We collected and analyzed quantitative and qualitative measures to answer our
research questions. For each research question, we describe our analysis
approach and results below. 
% We qualitatively analyzed conceptual models, statistical models, audio
% recordings, and open-ended survey responses. Whenever possible, we also
% quantified the frequency of characteristics in conceptual models and
% statistical models across participants. For the statistical models
% participants authored, we compared the AIC and BIC scores for matched pairs of
% the independent variable of interest. 


\subsubsection{\evalConceptualModels}
% Consistency within vs. across participants 
We qualitatively analyzed how consistent participants' conceptual models were
between conditions. We noted common challenges translating free-form conceptual
models into rTisane programs. We also thematically analyzed participant
transcripts and survey responses describing the influence of rTisane on their
conceptual modeling processes. 

% \subsubsection{\evalConceptualModelAuthoring}
% % To understand rTisane's influence on the conceptual modeling process, we
% % compared the ratings and thematically analyzed survey responses to questions
% % asking how participants decided what conceptual relationships to specify.
% At the end of Phases 2 and 3, we asked participants to rate and describe their
% experience specifying conceptual models without and with rTisane, respectively.
% In addition, we kept track of the conceptual modeling challenges participants
% vocalized and noted how participants overcame these challenges in-situ. We
% compared the survey responses, observed challenges, and observed approaches
% between Phases 2 and 3 to assess how rTisane influenced the conceptual modeling
% process. 

\subsubsection{\evalStatisticalModels}
We used AIC, BIC, and R-squared values to assess how well statistical models
authored with vs. without rTisane fit the data. We used rTisane to statistically
model and assess the influence of rTisane on AIC, BIC, and R-squared values.

We also thematically analyzed participants' reactions to the similarities,
differences, and surprises between statistical models. 

\todo{Add statistical models executed}
\todo{Add rTisane analysis script to supplemental material}

\subsubsection{\evalLearning}
Finally, we gauged participants' learning based on a thematic analysis of
open-ended survey interview answers at the end of the study. 

% Finally, we measured participants' learning based on survey scale and
% open-ended responses at the end of Phase 3. We also thematically analyzed
% participants' explanations about what they learned, if anything. 

\begin{comment}
\paragraph{\evalConceptualModelAuthoring What is the influence of the rTisane DSL on the process of authoring conceptual models?}
\begin{itemize}
\item Describe when analysts add/remove relationships from without rTisane to
with rTisane study phases
\item Count instances of times analysts say something about not realizing
conceptual relationships beforehand (limitation: rTisane is after initial
conceptual model so could be matter of time)
\item Summarize themes in survey responses to questions about awareness of
conceptual relationships
\item Qualitative analysis of the audio recordings?
\item Quantitatively analyze differences in NASA-TLX scores without and with
rTisane
\end{itemize}

\paragraph{\evalStatisticalModels How does rTisane impact the statistical models authored?}
There will be three statistical models for which to examine the following. 
\begin{itemize}
\item Quantify how many covariates were added/removed between without rTisane
and with rTisane
\item Describe which covariates are common, which are added/removed
\item Thematically analyze reasonsing for why specific covariates were
added/removed, 
\item Quantify how frequently participants chose specific family/link functions
\item Describe any other differences in statistical model form (e.g., linear vs.
polynomial; refuse linear model and use t-tests) and quantify frequency
\item Quantitatively compare AIC, BIC between without and with rTisane phases
(e.g., paired t-test?)
\item (surprise) Thematically analyze participants' reactions + survey questions
about surprise
\item (process) Quantitatively analyze differences in NASA-TLX scores without
and with rTisane 
\end{itemize}

\paragraph{\evalConceptualModels What is the influence of the rTisane DSL on conceptual models? Does using the rTisane DSL lead to qualitatively different conceptual models?}
\begin{itemize}
\item Describe conceptual models: Which variables and relationships are included
in both? one but not the other? (Why?)
\end{itemize}

\paragraph{\evalLearning Does using rTisane help researchers learn about authoring analyses?}
\begin{itemize}
\item Summarize themes of survey responses about what they learned
\end{itemize}

% Spread of conceptual models and statistical models

\subsection{Findings}
\end{comment}


==> archive/system.tex <==
\section{\tisane or Refining Tisane}

\subsection{Design goals}
\textbf{Deconstruct statistical constructs for clarity.}
\begin{itemize}
    \item Stick to causes. 
    \item As a result of sticking with only causes and explicitly introducing ambiguity in another step (see below), replace modified disjunctive criteria with d-separation rules. (Take ambiguity out of the reasoning process, createa an explicit step/stage for it)
    \item Unobserved tags: Associates --> causes with unobserved variables
    \item Moderates: 
    \item Trials
    \item Conditions
    \item Participant, and other generic Units
\end{itemize}
\textbf{Allow for conceptual ambiguity, make specificity optional.}
\begin{itemize}
    \item Phases of specifying: known vs. suspected (How to enforce phases?? syntactic diffrence?)
    \item Moderates: Ambiguity: DV, set of IVs
    \item TODO: Add opportunity to assess conceptual model - What does this look like? 
    \item TODO: Disambiguate with the user about how to treat ambiguous relationships
\end{itemize}
Future system should 
Action: Structured phases for capturing conceptual model, output a series of models to execute and interpret
-- Interpretation as a key question
\textit{Tradeoff ambiguity between analyst and system with statistical knowledge}

\textbf{Allow for conceptual ambiguity.}

\subsection{Specification language}
START with API docs:
https://github.com/emjun/rTisane/blob/refactor/API_OVERVIEW.md#measures 


\subsection{Conceptual model disambiguation}
What's interesting: 
Commentary: A way to facilitate thinking, reflection on relationships -- based on insight from exploratory story that people did not know how to specify structure/know what to do and needed guidance 
Commentary: Could be a form of reflection (tee up for summative eval)
What's interesting: Cycle breaking


\subsection{Statistical model disambiguation and Output}
\tisane leverages Tisane's statistical model derivation and disambiguation
process. 

The output is a script for executing a GLM for 

There are two outputs of the interactive compilation: (ii) an executable modeling script and (ii) a log of GUI
choices. To increase transparency of the
authoring process, Tisane provides a log of user selections in the GUI as
documentation, which the analyst can include in pre-registrations, for example. In the output script, Tisane includes code to fit the
model and plot residuals against fitted values in order to assess the
appropriateness of family and link functions, as is typical when examining
family and link functions. The output script also includes a comment explaining
what to look for in the plots and an online resource for further reading. Should
analysts revise their choice of family and link functions, they can re-generate
a script through the Tisane GUI.
